Dynamic Witnesses for Static Type Errors (or, Ill-Typed Programs Usually Go Wrong)

Static type errors are a common stumbling block for newcomers to typed functional languages. We present a dynamic approach to explaining type errors by generating counterexample witness inputs that illustrate how an ill-typed program goes wrong. First, given an ill-typed function, we symbolically execute the body to synthesize witness values that make the program go wrong. We prove that our procedure synthesizes general witnesses in that if a witness is found, then for all inhabited input types, there exist values that can make the function go wrong. Second, we show how to extend this procedure to produce a reduction graph that can be used to interactively visualize and debug witness executions. Third, we evaluate the coverage of our approach on two data sets comprising over 4,500 ill-typed student programs. Our technique is able to generate witnesses for around 85% of the programs, our reduction graph yields small counterexamples for over 80% of the witnesses, and a simple heuristic allows us to use witnesses to locate the source of type errors with around 70% accuracy. Finally, we evaluate whether our witnesses help students understand and fix type errors, and find that students presented with our witnesses show a greater understanding of type errors than those presented with a standard error message.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper we have demonstrated how to find \emph{dynamic} witnesses
to \emph{static} type errors.
%
Dynamic witnesses provide the user with more information than static
error messages, and enable the use of standard debugging techniques
to explore \emph{how} the program ``goes wrong''.
%
Our witness search produces general witnesses, precluding the
possiblity of a valid typing for the program.
%
We have shown a novel interactive visualization of the execution of
functional programs, which can be used to \emph{show} a novice how a
witness makes their program crash.
%
Our evaluation shows that our search is effective at finding witnesses
with a 87\% success rate, and that our jump-compressed traces
effectively hide boring details of the execution, with 90\% of the
benchmarks containing less than 10 jumps.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> evaluation-nanomaly.tex <==
\section{Evaluation: \nanomaly}
\label{sec:evaluation-nanomaly}
We have implemented our interactive semantics for the pure subset of
\ocaml with a web-based visualization of the generated traces in a tool
called \nanomaly.
%
It takes as input an \ocaml program and a function to check, searches
for a witness as described in \S~\ref{sec:searching-witness}, and
produces as output an interactive trace of the (possibly buggy)
execution~\footnote{If no witness could be found we simply return a trace
  of the last attempt.}.

We have not really (\ES{huh?}) evaluated our prototype of \nanomaly in two phases:
%
\begin{enumerate}
\item We investigate the \emph{complexity} of the generated traces by various size metrics.
\item We investigate the \emph{usefulness} of the generated traces compared to the standard compiler errors by performing an A/B study.
\end{enumerate}

\subsection{Trace Complexity}
\label{sec:trace-complexity}
For each of the ill-typed programs from \S~\ref{sec:eval-witness} for
which we could find a witness, we measure the complexity of the
generated trace according to the following metrics:
%
\begin{enumerate}
\item The number of single-step reductions along the path from the
  witness to the stuck term. This can be thought of as a worst-case
  complexity, \ie ``How big is the fully-expanded trace?''
\item The number forward (or backward) jumps that can be taken along the
  path from the witness to the stuck term. These abstract many details
  of the computation that are often uninteresting or irrelevant to the
  explanation.
\item \ES{others?}
\end{enumerate}
%
\begin{figure*}[t]
\centering
% \includegraphics[width=\linewidth]{trace_size.pdf}
\begin{minipage}{0.49\linewidth}
\includegraphics[width=\linewidth]{trace_size_step.pdf}
\end{minipage}
\begin{minipage}{0.49\linewidth}
\includegraphics[width=\linewidth]{trace_size_jump.pdf}
\end{minipage}
\caption{Complexity of the generated traces.}
\label{fig:results-complexity}
\end{figure*}
%
The results of the experiment are summarized in
Figure~\ref{fig:results-complexity}.
%
The average number of single-step reductions is XX with a minimum of XX
and a maximum of XX. The average number of jumps is YY with a minimum of
YY and a maximium of YY.

\subsection{User Study}
\label{sec:user-study}
We also performed an A/B study at the University of Virginia (IRB
\#XXXX). 
%
Participants were recruited from the graduate-level Programming
Languages course CSYYY, with the possibility of winning a \$50 gift
certificate upon completion.
%
We selected a random sample of nine ill-typed programs from our
benchmark dataset and from submissions to our public-facing demo of
\nanomaly.
%
For each program, we presented participants with the program and
alternatingly, either \ocaml's type error message or our interactive
visualization of a preset trace.
%
In order to alleviate any potential bias in problem selection, we also
alternated whether participants began with \ocaml or \nanomaly.
%
Participants were asked to identify the \emph{source} of the error,
\emph{explain} the error, and finally \emph{fix} it.

We collected the time taken for each problem and recruited a colleague
to grade the submissions, hiding whether a given solution came from the
\ocaml or \nanomaly group.

\paragraph{Results}
\label{sec:study-results}
\ES{TODO!}


==> evaluation-witness.tex <==
\section{Evaluation: Recasting Type Errors as Runtime Errors}
\label{sec:eval-witness}
%
The immediate question is ``What fraction of type errors admit
witnesses?''
%
To answer this question we implemented a prototype of our search
procedure for the pure subset of \ocaml, \ie \lang extended with
algebraic datatypes and records. 
%
In our implementation we instantiated \gensym with a simple random
generation of values, which we will show is more than sufficient for the
majority of type errors.
%
We evaluated our implementation of two sets of known-bad programs, \ie
programs that were rejected by the \ocaml compiler because of a type
error.
%
The first dataset comes from the Spring 2014 undergraduate Programming
Languages course at UC San Diego (IRB \#140608). 
%
We recorded each interaction with the \ocaml top-level system over the
course of the first three assignments, from which we extracted XXXX
distinct, ill-typed \ocaml programs.
%
The second dataset -- widely used in the literature -- comes from a
similar course at the University of
Washington~\cite{Lerner2006-pj}, from which we extracted 284
ill-typed programs.

We ran our search algorithm on each program with the entry point set to
the function that \ocaml had identified as containing a type error. 
%
Due to the possibility of non-termination we set a limit on the number
of reductions to perform, increasing in 500-step increments from 500
steps to 3,000 steps total.
%
We also added a na\"ive check for infinite recursion; at each recursive
function call we check whether the new arguments are identical to the
current arguments.
%
If so, the function cannot possibly terminate and we report an error.
%
While not a \emph{type error}, infinite recursion is still a clear bug
in the program, and thus valuable feedback for the user.

\begin{figure}[t]
\centering
\begin{minipage}{\linewidth}
\includegraphics[width=\linewidth]{coverage.pdf}
\end{minipage}
\begin{minipage}{\linewidth}
\includegraphics[width=\linewidth]{distrib.pdf}
\end{minipage}
% \vspace{-8ex}
\caption{Experimental results. Our random search successfully finds
  witnesses for over 85\% of the programs at the lowest timeout and
  improves slightly to 88\% at the next level. In both datasets we
  detect actual type errors about 82\% of the time, unbound variables or
  constructors 3-4\% of the time, and diverging loops 2-3\% of the
  time. For the remaining 11-12\% of the programs we are unable to
  provide any useful feedback. 
}
\label{fig:results-witness}
\end{figure}

\paragraph{Results}
\label{sec:results-witness}
The results of our experiments are summarized in
Figure~\ref{fig:results-witness}.
%
In both datasets our tool was able to find a witness for at least XX\%
of the programs.
%
Interestingly, while the vast majority of witnesses corresponded to a
type-error, as expected, X\% triggered an unbound variable error and X\%
triggered an infinite recursion error.
%
XX programs were deemed safe and XX timed out even at 3,000 steps, \ie
we could not provide any useful feedback for XX\% of the total programs.
%
While a more advanced search procedure, \eg dynamic-symbolic execution,
could likely trigger more of the type errors, our experiments show that
type errors are coarse enough (or that novice programs are \emph{simple}
enough) that these techniques are not necessary.



% \begin{itemize}
% \item benchmarks: our data + seminal data
% \item both cases: \textbf{random} search sufficient to trigger runtime crash in 80\% of programs
% \item how many of the ``safe'' programs are actually safe??
% \end{itemize}


==> gallery.tex <==
\section{The Advantage Of Traces}
\label{sec:advantage-traces}
Finally, having shown that \toolname produces small traces in an
efficient manner, let us discuss the explanatory power of traces
compared with typical type error messages. In this section we will
present a qualitative evaluation of \toolname's jump-compressed traces
on a series of examples drawn from real student programs in the
\ucsdbench dataset. For each example we will present the code, a
jump-compressed trace produced by \toolname, and the type error produced
by the \ocaml compiler.

\begin{figure*}[ht]
\centering
\begin{minipage}{0.49\linewidth}
\centering
\begin{ecode}
let rec sqsum xs = match xs with
  | [] -> 0
  | h::t -> __(sqsum t)__ @ (h * h)
\end{ecode}
% File "sqsum.ml", line 3, characters 12-21:
\begin{verbatim}
Error: This expression has type
         int
       but an expression was expected of type
         'a list
\end{verbatim}
\end{minipage}
\begin{minipage}{0.49\linewidth}
\centering
\includegraphics[height=125px]{sqsum.png}
\end{minipage}
\caption{\texttt{sqsum xs} should square each element of \texttt{xs} and
  then compute the sum of the result, but the student has used the
  list-append operator |@| instead of \texttt{+} to compute the
  sum. \ocaml blames the recursive call \texttt{sqsum t} (underlined
  above) for being an \texttt{int} instead of a \texttt{list}.
  \toolname's jump-compressed trace draws the eye to the
  entire term \texttt{0 }|@|\texttt{ 1}.}
\label{fig:trace-sqsum}
\end{figure*}

\begin{figure*}[ht]
\centering
\begin{minipage}{0.49\linewidth}
\centering
\begin{ecode}
let rec sumList xs = match xs with
  | []    -> []
  | y::ys -> y + __sumList ys__
\end{ecode}
% File "sumList.ml", line 3, characters 17-27:
\begin{verbatim}
Error: This expression has type
         'a list
       but an expression was expected of type
         int
\end{verbatim}
\end{minipage}
\begin{minipage}{0.49\linewidth}
\centering
\includegraphics[height=125px]{sumlist.png}
\end{minipage}
\caption{\texttt{sumList xs} should sum the elements of \texttt{xs}, but
  the student has returned \texttt{[]} in the base case instead of
  \texttt{0}. \ocaml deduces from the base case that \texttt{sumList}
  must return a \texttt{list} and thus blames the recursive call on line
  3 for producing a \texttt{list} instead of an  \texttt{int}.
  \toolname's jump-compressed trace highlights the clash
  between the \texttt{[]} and the \texttt{+}, but also demonstrates in
  the third step that \texttt{sumList []} reduces to \texttt{[]}, which
  clarifies that the conflict is between the base case and recursive
  case.}
\label{fig:trace-sumlist}
\end{figure*}

\begin{figure*}[ht]
\centering
\begin{minipage}{0.49\linewidth}
\centering
\begin{ecode}
let append xs ys = match xs with
  | []   -> ys
  | h::t -> h :: __t__ :: ys
\end{ecode}
% File "append.ml", line 3, characters 17-18:
\begin{verbatim}
Error: This expression has type
         'a list
       but an expression was expected of type
         'a
       The type variable 'a occurs inside 'a list
\end{verbatim}
\end{minipage}
\begin{minipage}{0.49\linewidth}
\centering
\includegraphics[height=75px]{append.png}
\end{minipage}
\caption{\texttt{append xs ys} should concatenate the two input lists,
  but the student has tried to cons the tail of \texttt{xs} onto
  \texttt{ys} instead of making a recursive call to \texttt{append}.
  \ocaml blames \texttt{t} on line 3 for being a \texttt{'a list}
  instead of a \texttt{'a}, prompting an \emph{occurs-check}
  error. \toolname shows, more concretely, that \texttt{[] :: [2]} gets
  stuck because lists are homogeneous and \texttt{[]} is not an
  \texttt{int}.}
\label{fig:trace-append}
\end{figure*}

\begin{figure*}[ht]
\centering
\begin{minipage}{0.49\linewidth}
\centering
\begin{ecode}
let rec wwhile (f,b) =
  match f with
  | (z, false) -> z
  | (z, true)  -> wwhile (f, z)

let f x =
  let xx = x * x in
  (xx, (xx < 100))

let _ = wwhile (__f__, 2)
\end{ecode}
% File "wwhile.ml", line 10, characters 16-17:
\begin{verbatim}
Error: This expression has type
         int -> int * bool
       but an expression was expected of type
         'a * bool
\end{verbatim}
\end{minipage}
\begin{minipage}{0.49\linewidth}
\centering
\includegraphics[height=150px]{wwhile.png}
\end{minipage}
\caption{\texttt{wwhile (f, b)} should repeatedly apply the function
  \texttt{f} to the first element of its result pair, starting with the
  initial input \texttt{b}, until the second element is \texttt{false}.
  Unfortunately, the student has forgotten to apply \texttt{f} at all on
  line 2, and just matches it directly against a pair. This faulty
  definition of \texttt{wwhile} still typechecks however, and \ocaml
  thus blames the \emph{call-site} on line 10. \toolname makes no
  assumptions about the input code and quickly draws the eye to the true
  error, the \texttt{match} expression, and highlights the conflict in
  matching a function against a pair pattern.}
\label{fig:trace-wwhile}
\end{figure*}














%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> gallery2.tex <==


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> interactive.tex <==
\section{Explaining Type Errors With Traces}
\label{sec:interactive}

A trace, on its own, is too detailed to be
a good explanation of the type error. One approach
is to use the witness input to step through the
program with a \emph{debugger} to observe how
the program evolves.
%
This route is problematic for two reasons.
%
First, existing debuggers and interpreters for
typed languages (\eg\ \ocaml) typically require
a type-correct program as input.
%
Second, we wish to have a quicker way to get
to the essence of the error, \eg\ by skipping
over irrelevant sub-computations, and focusing
on the important ones.

In this section we present a novel way to debug executions.
%
First, we develop a notion of a \emph{reduction graphs}
and extend our semantics with a form of \emph{tracing}
so that they incrementally collect the edges
in the graph (\S~\ref{sec:inter-semant}).
%
Next, we express a set of common \emph{interactive debugging}
steps as graph traversals (\S~\ref{sec:traversing-graph}), yielding
an novel interactive debugger that allows the user
to effectively visualize \emph{how} the program goes (wrong).

\subsection{Tracing Semantics}
\label{sec:inter-semant}
%
% \begin{figure*}[t]
% %% \relDescription{Computing Sub-Terms}
% %% \begin{gather*}
% %% \begin{array}{lcl}
% %% \subtermssym                 & \dcolon & e \to \tr \\
% %% \subterms{\eapp{e_1}{e_2}}   & \defeq & \subterm{\eapp{e_1}{e_2}}{e_1}; \subterm{\eapp{e_1}{e_2}}{e_2} \\
% %% \subterms{\eplus{e_1}{e_2}}   & \defeq & \subterm{\eplus{e_1}{e_2}}{e_1}; \subterm{\eplus{e_1}{e_2}}{e_2} \\
% %% \subterms{\eif{e_1}{e_2}{e_3}}   & \defeq & \subterm{\eif{e_1}{e_2}{e_3}}{e_1}; \\
%                                 %% &        & \subterm{\eif{e_1}{e_2}{e_3}}{e_2}; \\
%                                 %% &        & \subterm{\eif{e_1}{e_2}{e_3}}{e_3} \\
% %% \subterms{\elet{x}{e_1}{e_2}}   & \defeq & \subterm{\elet{x}{e_1}{e_2}}{e_1}; \\
%                                 %% &        & \subterm{\elet{x}{e_1}{e_2}}{e_2} \\
% %% \subterms{\efun{x}{e}}       & \defeq & \subterm{\efun{x}{e}}{e} \\
% %% \subterms{e}                 & \defeq & \bullet
% %% \end{array}
% %% \end{gather*}
% \judgementHead{Traced Evaluation}{\stepg{e}{\su}{\tr}{e}{\su}{\tr}}
% \begin{gather*}
% \inference[\recontext]
%   {\stepg{e}{\su}{\tr}{e'}{\su'}{\tr'}}
%   {\stepg{C[e]}{\su}{\tr}{C[e']}{\su'}{\singlestep{C[e]}{C[e']}; \tr'}}
% \\ \\
% \inference[\reappgood]
%   {\pair{\efun{x}{e}}{\su'} = \force{v_1}{\tfun{\thole{}}{\thole{}}}{\su}}
%   {\stepg{\eapp{v_1}{v_2}}{\su}{\tr}
%          {e\sub{x}{v_2}}{\su'}{\singlestep{\eapp{v_1}{v_2}}{e\sub{x}{v_2}}; \tr}}
% \\ \\
% \inference[\reappbad]
%   {\pair{\stuck}{\su'} = \force{v_1}{\tfun{\thole{}}{\thole{}}}{\su}}
%   {\stepg{\eapp{v_1}{v_2}}{\su}{\tr}{\stuck}{\su'}{\singlestep{\eapp{v_1}{v_2}}{\stuck}; \tr}}
% \end{gather*}
% \caption{A selection of the operational semantics from
%   Figure~\ref{fig:operational}, extended to collect a full reduction
%   graph.}
% \label{fig:interactive}
% \end{figure*}

\paragraph{Reduction Graphs}
%
A \emph{steps-to} edge is a pair of expressions \singlestep{e_1}{e_2}, which
intuitively indicates that $e_1$ reduces, in a single step, to $e_2$.
%
%A \emph{sub-term} edge is a pair of expressions \subterm{e_1}{e_2}, which
%intuitively indicates that $e_1$ contains $e_2$ as a sub-expression.
%
A \emph{reduction graph} is a set of steps-to edges:
$$\tr ::= \bullet \spmid \singlestep{e}{e}; \tr$$  %% \spmid \subterm{e}{e}; \tr$$

\paragraph{Tracing Semantics}
%
We extend the transition relation (\S~\ref{sec:semantics}) to
collect the set of edges corresponding to the reduction graph.
%
Concretely, we extend the operational semantics to
a relation of the form $\stepg{e}{\vsu}{\tsu}{\tr}{e'}{\vsu'}{\tsu'}{\tr'}$
where $\tr'$ collects the edges of the transition.

\paragraph{Collecting Edges}
%
Next, we describe the general recipe for extending a transition
rule to collect edges.
%
The general recipe for collecting steps-to edges is
to record the consequent of each original rule in the
trace. That is, each original judgment \step{e}{\vsu}{\tsu}{e'}{\vsu'}{\tsu'}
becomes \stepg{e}{\vsu}{\tsu}{\tr}{e'}{\vsu'}{\tsu'}{\singlestep{e}{e'}; \tr}.
%
As the translation is mechanical, we provide a selection of examples
in Figure~\ref{fig:interactive}.
% As the translation is mechanical, we will not discuss it further.

%%% The sub-term edges are delegated to a helper function \subtermssym\
%%% which adds edges from an expression to each of its
%%% \emph{immediate} sub-expressions.
%%% %
%%% We collect \subtermssym\ edges after each transition,
%%% to get the following template for the small-step relation:
%%% \[
%%% \stepg{e}{\vsu}{\tr}{e'}{\vsu'}{\singlestep{e}{e'}; \subterms{e'}; \tr}
%%% \]


\subsection{Interactive Debugging}
\label{sec:traversing-graph}

Next, we show how to build a visual interactive debugger
from the traced semantics, by describing the visualization
\emph{state} \ie\ what the user sees at any given moment,
the set of \emph{commands} available to user and what
they do, and finally how we use a command to \emph{update}
the visualization state. In what follows, for clarity of
exposition, we assume we have a (global) trace:
$\stepg{e_0}{\emptysu}{\emptysu}{\bullet}{e_n}{\vsu}{\tsu}{\tr}$, where
$e_0$ and $e_n$ are the \emph{initial} and \emph{final}
expressions respectively.

\paragraph{Visualization State}
%
A \emph{visualization state} $\vstate$ is a \emph{directed graph}
whose vertices are expressions and whose edges are such
that each vertex has at most one predecessor and at most one
successor. In other words, the visualization state looks
like a set of linear lists of expressions as shown in
Figure~\ref{fig:nanomaly-factorial}.
%
The \emph{initial state} is the graph containing a single
edge linking the initial and final expressions.

\paragraph{Visualization Context}
%
The \emph{visualization context} of each expression $e$
in the visualization state $\vstate$ is the (unique) linear chain
in which the expression $e$ belongs.
%
We write $\vroot{\vstate}{e}$ for the \emph{first} (or root)
expression appearing in the visualization context of $e$ in
$\vstate$.

\paragraph{Commands}
Our debugger supports the following \emph{commands}, each of which
is parameterized by a single expression (vertex) selected from the
(current) visualization state:
%
\begin{itemize}
%
\item \stepforwardsym, \stepbackwardsym:
      show the result of a single step forward or backward respectively,
%
\item \jumpforwardsym, \jumpbackwardsym:
      show the result of taking multiple steps (a \emph{``big''} step)
      upto the first beta-reduction forward or backward respectively,
%
\item \stepintosym:
      show the result of stepping into a function call in a sub-term,
      isolating it from the context,

\item \stepoversym:
      show the result of skipping over a function call in a sub-term.
\end{itemize}

\input{traversals_new.tex}

\paragraph{Update}
%
Figure~\ref{fig:traversing-graph} shows
how we compute the \emph{next} expression
(to be added to the visualization state)
given the current visualization state
$\vstate$, command $\cmd$ and selected
expression $e$.
%
It is straightforward to then \emph{update}
the visualization graph by adding the new
term before (resp.\ after) the selected
expression $e$ if the command was a step
or jump forward (resp.\ backward), or
to create a new visualization context
if the command was $\stepintosym$.

%%% and \updState{\vstate}{\cmd}{e} then updates the graph
%%% by inserting the new expression appropriately, using
%%% one of the following graph manipulating functions:
%%% %
%%% \putBefore{\vstate}{e}{e'} (resp. \putAfter{\vstate}{e}{e'})
%%% returns the modified version of \vstate\ where $e'$ is the
%%% immediate predecessor of $e$ (resp.\ the immediate successor of $e$);
%%% %
%%% \putRoot{\vstate}{e}{e'} returns the modified version of \vstate
%%% extended with a new root vertex $e$ with successor $e'$.
%%% %
%%% @getNext vs e@ returns the immediate successor of @e@ in $\tr$.
%%% %
%%% @getPrev vs e@ computes the path @p@ between @e@ and its immediate
%%% predecessor in the current visualization, and then returns @e@'s immediate
%%% predecessor along @p@.
%%% %
%%% @getSubterms vs e@ traverses the sub-term edges to decompose an
%%% expression into a list of sub-expressions paired with their context.
%%% %
%%% @applyCtx vs e ctx@ applies @ctx@ to @e@, traversing the sub-term edges
%%% in reverse to find the super-term of @e@.
%%% %
%%% \hbox{@findApp vs e@} builds on top of @getSubterms@ to find the first
%%% application sub-term (if any), \ie the first sub-term that looks like
%%% $\eapp{v_1}{v_2}$.
%%% %
%%% @findVal vs e@ traverses the single-step edges to find the final value
%%% that @e@ reduces to.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fac-steps-new.png}
\caption{A sequence of interactions with the trace of
  \texttt{fac 1}. The stuck term is red, in each node the redex is
  highlighted. Thick arrows denote a multi-step transition, thin arrows
  denote a single-step transition. We start in step 1. In step 2 we jump
  forward from the witness to the next function call. In step 3 we step
  into the recursive \texttt{fac 0} call, which spawns a new ``thread''
  of execution. In step 4 we take a single step forward from
  \texttt{fac 0}.}
\label{fig:nanomaly-factorial}
\end{figure}


==> nanomaly.tex <==
\section{Our Implementation: \nanomaly}
\label{sec:impl-nanomaly}
We have implemented our interactive semantics for the pure subset of
\ocaml with a web-based visualization of the generated traces in a tool
called \nanomaly.
%
It takes as input an \ocaml program and a function to check, searches
for a witness as described in \S~\ref{sec:searching-witness}, and
produces as output an interactive trace of the (possibly buggy)
execution~\footnote{If no witness could be found we simply return a trace
  of the last attempt.}.
%
We initially display a big-step reduction, \ie the source term followed
by the stuck term (or the final value).
%
The user can then progressively fill in the hidden steps of the
computation by selecting a visible term and choosing one of the
applicable traversal strategies -- described in
\S~\ref{sec:traversing-graph} -- to insert another term into the
visualization.

A sample interaction of the student program in
Figure~\ref{fig:palindrome} can be seen in
Figure~\ref{fig:nanomaly-palindrome}.
%
The initial state of the visualization tells us that the witness is
@palindrome []@, and that after some number of steps -- the thick arrow
denotes a multi-step transition -- we try to compare a function to a
list, which is not allowed in \ocaml.
%
Based on our semantics for \lang one would expect the final state to be
the \stuck term, but in practice we simply halt execution at the point
where an expression would transition to \stuck, as this final state is
more informative.
%
Note also that the equality test is colored black while the contextual
if-expression is faded out, this tells the user that the program got
stuck while trying to evaluate the sub-expression.

Upon seeing the stuck term, one might wonder where the @function@
came from.
%
To investigate we select the stuck term and click the ``jump backward''
button to search backwards from the stuck term for the most recent
function call, which brings us to @listReverse [] = w@, in the same
context as before.
%
Uncontent with the explanation so far, we ``step forward'' twice from
the @listReverse []@ term, bringing us to @helper [] = w@.
%
At this point it is clear that the @helper@ function is not defined
correctly, we have supplied it with the single argument we expected and
yet it still returned a @function@.

The problem is that the @function@ keyword in \ocaml defines an
anonymous function that takes a single argument and immediately does a
case-analysis without giving the argument a name.
%
The solution is to replace @function@ with an explicit @match xs with@
-- naming the value we wish to case-analyse.
%
After applying our fix, \nanomaly -- and more importantly \ocaml --
decide that @listReverse@ is safe to run.
\ES{these last few paragraphs probably belong in the overview}
%
\begin{figure}[t]
\centering
\begin{code}
  let listReverse l =
    let rec helper xs = function
      | [] -> xs
      | hd::tl -> helper (hd :: xs) tl
    in helper []

  let palindrome w =
    if listReverse w = w
    then true
    else false
\end{code}
\caption{Ill-typed \texttt{palindrome} function. The error lies in the
  use of the \texttt{function} construct which introduces an extra,
  undesired lambda abstraction, but manifests itself in the equality
  test on line XX. The fix is to replace \texttt{function} with
  \texttt{match xs with}. \ES{I think we should use this example in the
    intro/overview, leaving it here for now until they exist..}}
\label{fig:palindrome}
\end{figure}
%
\begin{figure}[t]
% \centering
Initial state: \\
\includegraphics[width=\linewidth]{palindrome} \\
After ``jumping backward'' from the stuck term: \\
\includegraphics[width=\linewidth]{palindrome2} \\
After ``stepping forward'' twice from @listReverse []@: \\
\includegraphics[width=\linewidth]{palindrome3} \\
\caption{Sample interaction}
\label{fig:nanomaly-palindrome}
\end{figure}

% !TEX root = main.tex


==> traversals.tex <==
\begin{figure}[t]
\centering
% \begin{minipage}{0.49\linewidth}
\begin{mcode}
 putBefore :: VState -> Expr -> Expr -> VState
 putAfter  :: VState -> Expr -> Expr -> VState
 putRoot   :: VState -> Expr -> Expr -> VState

 getNext   :: VState -> Expr -> Maybe Expr
 getPrev   :: VState -> Expr -> Maybe Expr

 getSubterms :: VState -> Expr -> [(Expr,Ctx)]
 applyCtx    :: VState -> Expr -> Ctx -> Expr
 
 findApp :: VState -> Expr -> Maybe (Expr,Ctx)
 findVal :: VState -> Expr -> Expr
 
 data Cmd = StepForward | StepBack
          | JumpForward | JumpBack
          | StepInto    | StepOver
\end{mcode}
% data \ctx
\caption{Graph manipulation and traversal API.}
\label{fig:graph-api}
\end{figure}
% \end{minipage}
% \begin{minipage}{0.49\linewidth}
\begin{figure}[t]
\begin{mcode}
findExpr :: VState -> Cmd -> Expr -> Maybe Expr
findExpr v c e = case c of
  StepForward -> getNext v e
  StepBack    -> getPrev v e
  JumpForward -> case findExpr v StepForward e of
    $\eapp{v_1}{v_2}$ -> Just ($\eapp{v_1}{v_2}$)
    e'   -> findExpr v c e'
  JumpBack    -> case findExpr v StepBack e of
    $\eapp{v_1}{v_2}$ -> Just ($\eapp{v_1}{v_2}$)
    e'   -> findExpr v c e'
  StepInto    -> findApp v e
  StepOver    -> case findApp v e of
    Nothing       -> Nothing
    Just (e', cx) -> applyCtx v (findVal v e') cx

updState :: VState -> Cmd -> Expr -> Maybe VState
updState v c e = case findExpr v c e of
  Nothing -> Nothing
  Just e' -> Just (*\$*) case c of
    StepForward -> putAfter  v e e'
    StepBack    -> putBefore v e e'
    JumpForward -> putAfter  v e e'
    JumpBack    -> putBefore v e e'
    StepInto    -> putRoot   v e' (findVal v e') 
    StepOver    -> putAfter  v e e'
\end{mcode}
% \end{minipage}
% \[
% \begin{array}{lcl}
% \stepforward{G}{p}{e_i}  &\defeq& \left\{\begin{array}{ll}
%     e_j, & \text{where } \singlestep{e_i}{e_j} \in G
%                          \end{array}\right\} \\ \\
% \stepbackward{G}{p}{e_i}  &\defeq& \left\{\begin{array}{ll}
%     e_j, & \text{where } \singlestep{e_j}{e_i} \in G \text{ and } e_j \in p
%                          \end{array}\right\} \\ \\
% \jumpforward{G}{p}{e_i} &\defeq& \text{let } e_j = \stepforward{G}{p}{e_i} \text{ in }
%                          \left\{\begin{array}{ll}
%                          e_j, & \text{if } e_j = \eapp{v_1}{v_2} \\
%                          \jumpforward{G}{p}{e_{j}}, & \text{otherwise}
%                          \end{array}\right\} \\ \\
% \jumpbackward{G}{p}{e_i} &\defeq& \text{let } e_j = \stepbackward{G}{p}{e_i} \text{ in }
%                          \left\{\begin{array}{ll}
%                          e_j, & \text{if } e_j = \eapp{v_1}{v_2} \\
%                          \jumpbackward{G}{p}{e_{j}}, & \text{otherwise}
%                          \end{array}\right\} \\ \\
% \stepinto{G}{p}{e_i} &\defeq& \left\{\begin{array}{ll}
%                          e\sub{x}{v_2}, & \text{if } e_i = C[\eapp{v_1}{v_2}] \text{ and } \singlestep{\eapp{v_1}{v_2}}{e\sub{x}{v_2}}
%                          \end{array}\right\} \\ \\
% \stepover{G}{p}{e_i} &\defeq& \left\{\begin{array}{ll}
%                          C[v], & \text{if } e_i = C[\eapp{v_1}{v_2}] \text{ and } \multistep{\eapp{v_1}{v_2}}{v}
%                          \end{array}\right\}
% \end{array}
% \]
\caption{Rules for updating the reduction graph given a command and a selected expression. \texttt{updState} returns \texttt{Nothing} if the command was not applicable. % \stepintosym and \stepoversym require a traversal of the
  % sub-term edges to decompose $e_i$ into the target expression
  % \eapp{v_1}{v_2} and the context $C$.  \ES{these rules are quite ugly and waste space..}
}
\label{fig:traversing-graph}
\end{figure}


==> traversals_new.tex <==
\begin{figure*}[t]
\[
\begin{array}{lcl}
\stepforward{\vstate}{e}  & \defeq
  & e' \quad \mbox{where } \singlestep{e}{e'} \in \tr \\ \\

\stepbackward{\vstate}{e} & \defeq
  & e' \quad \mbox{where } \singlestep{e'}{e} \in \tr \mbox{ and } e' \in \vpath{\vstate}{e} \\ \\

\jumpforward{\vstate}{e} & \defeq
  & \begin{cases}
    e'                         & \mbox{if } e' = \eapp{v}{v'} \\
    \jumpforward{\vstate}{e'}  & \text{otherwise}
    \end{cases}
    \mbox{\qquad where } e' = \stepforward{\vstate}{e} \\ \\

\jumpbackward{\vstate}{e} & \defeq
  & \begin{cases}
    e'                         & \mbox{if } e' = \eapp{v}{v'} \\
    \jumpbackward{\vstate}{e'} & \text{otherwise}
    \end{cases}
    \mbox{\qquad where } e' = \stepbackward{\vstate}{e} \\ \\

\stepinto{\vstate}{e} & \defeq
  & e'\sub{x}{v'} \quad \mbox{if } e = C[\eapp{v}{v'}] \mbox{ and } \singlestep{\eapp{v}{v'}}{e'\sub{x}{v'}}  \\ \\

\stepover{\vstate}{e} & \defeq
  & C[v''] \quad \mbox{if } e = C[\eapp{v}{v'}] \mbox{ and } \multistep{\eapp{v}{v'}}{v''} \in \tr \\[0.25in]

\vpath{\vstate}{e} & \defeq
  & \{e' \spmid \multistep{\vroot{\vstate}{e}}{e'} \in \tr
                \mbox{ and }
                \multistep{e'}{e} \in \tr \} \\[0.15in]
\end{array}
\]
\caption{Rules for computing the \emph{next} term given a
         visualization state $\vstate$, selected term $e$
         and command.}
\label{fig:traversing-graph}
\end{figure*}


==> traversals_old.tex <==
\begin{figure*}[t]
\[
\begin{array}{lcl}
\stepforward{G}{p}{e_i}  &\defeq& \begin{array}{ll}
    e_j, & \text{where } \singlestep{e_i}{e_j} \in G
                         \end{array}\right\} \\ \\
\stepbackward{G}{p}{e_i}  &\defeq& \left\{\begin{array}{ll}
    e_j, & \text{where } \singlestep{e_j}{e_i} \in G \text{ and } e_j \in p
                         \end{array}\right\} \\ \\
\jumpforward{G}{p}{e_i} &\defeq& \text{let } e_j = \stepforward{G}{p}{e_i} \text{ in }
                         \left\{\begin{array}{ll}
                         e_j, & \text{if } e_j = \eapp{v_1}{v_2} \\
                         \jumpforward{G}{p}{e_{j}}, & \text{otherwise}
                         \end{array}\right\} \\ \\
\jumpbackward{G}{p}{e_i} &\defeq& \text{let } e_j = \stepbackward{G}{p}{e_i} \text{ in }
                         \left\{\begin{array}{ll}
                         e_j, & \text{if } e_j = \eapp{v_1}{v_2} \\
                         \jumpbackward{G}{p}{e_{j}}, & \text{otherwise}
                         \end{array}\right\} \\ \\
\stepinto{G}{p}{e_i} &\defeq& \left\{\begin{array}{ll}
                         e\sub{x}{v_2}, & \text{if } e_i = C[\eapp{v_1}{v_2}] \text{ and } \singlestep{\eapp{v_1}{v_2}}{e\sub{x}{v_2}}
                         \end{array}\right\} \\ \\
\stepover{G}{p}{e_i} &\defeq& \left\{\begin{array}{ll}
                         C[v], & \text{if } e_i = C[\eapp{v_1}{v_2}] \text{ and } \multistep{\eapp{v_1}{v_2}}{v}
                         \end{array}\right\}
\end{array}
\]
\caption{Rules for updating the reduction graph given a command and a selected expression. \texttt{updState} returns \texttt{Nothing} if the command was not applicable. % \stepintosym and \stepoversym require a traversal of the
  % sub-term edges to decompose $e_i$ into the target expression
  % \eapp{v_1}{v_2} and the context $C$.  \ES{these rules are quite ugly and waste space..}
}
\label{fig:traversing-graph}
\end{figure*}

